Radio imaging of gravitationally lensed radio-quiet quasars

We present 6-GHz Very Large Array radio images of 70 gravitational lens systems at 300-mas resolution, in which the source is an optically-selected quasar, and nearly all of which have two lensed images. We find that about in half of the systems (40/70, with 33/70 secure), one or more lensed images are detected down to our detection limit of 20microJy/beam, similar to previous investigations and reinforcing the conclusion that typical optically-selected quasars have intrinsic GHz radio flux densities of a few microJy ($\sim10^{23}$WHz$^{-1}$ at redshifts of 1--2). In addition, for ten cases it is likely that the lensing galaxies are detected in the radio. Available detections of, and limits on the far-infrared luminosities from the literature, suggest that nearly all of the sample lie on the radio-FIR correlation typical of star-forming galaxies, and that their radio luminosities are at least compatible with the radio emission being produced by star formation processes. One object, WISE2329$-$1258, has an extra radio component that is not present in optical images, and is difficult to explain using simple lens models. In-band spectral indices, where these can be determined, are generally moderately steep and consistent with synchrotron processes either from star-formation/supernovae or AGN. Comparison of the A/B image flux ratios at radio and optical wavelengths suggests a 10 per cent level contribution from finite source effects or optical extinction to the optical flux ratios, together with sporadic larger discrepancies that are likely to be due to optical microlensing.

==> dojmfit_output_casa <==
  J0011$-$0845 & 00:11:20.24 $-$08:45:51.5  &     23$\pm$5  & -  & - \\
    J0013+5119 & 00:13:23.54 +51:19:05.9  &    192$\pm$4  &    261$\pm$4  &    302$\pm$4 \\
  PSJ0028+0631 & 00:28:22.49 +06:31:54.1 &      &      &     \\
    J0102+2445 & 01:02:47.22 +24:45:15.8  &     19$\pm$4  & -  & - \\
SDSSJ0114+0722 & 01:14:38.35 +07:22:28.9 &      &      &     \\
  J0124$-$0033 & 01:24:57.46 $-$00:33:11.5 &      &      &     \\
  J0140$-$1152 & 01:40:03.00 $-$11:52:19.4  &     20$\pm$5  & -  & - \\
  PSJ0140+4107 & 01:40:49.01 +41:07:59.9  &     14$\pm$4  &     24$\pm$4  & - \\
  J0146$-$1133 & 01:46:32.86 $-$11:33:38.9  &     32$\pm$5  &     26$\pm$5  & - \\
    J0203+1612 & 02:03:59.40 +16:12:08.6  &     46$\pm$4  & -  & - \\
    J0228+3953 & 02:28:11.10 +39:53:07.3  &     42$\pm$5  &     71$\pm$5  & - \\
 HE0230$-$2130 & 02:32:33.19 $-$21:17:25.7  &     30$\pm$5  &     48$\pm$5  &     30$\pm$5 \\
  J0235$-$2433 & 02:35:27.41 $-$24:33:13.7  &     26$\pm$6  &     32$\pm$6  & - \\
DESJ0245$-$0556 & 02:45:25.56 $-$05:56:59.6  &     42$\pm$5  &     27$\pm$5  & - \\
  J0246$-$1845 & 02:46:12.20 $-$18:45:05.0  &     80$\pm$7  &     45$\pm$7  & - \\
SDSSJ0246$-$0825 & 02:46:34.09 $-$08:25:36.1 &      &      &     \\
SDSSJ0256+0153 & 02:56:40.73 +01:53:29.4  &    114$\pm$5  & -  & - \\
DESJ0407$-$1931 & 04:07:53.79 $-$19:31:22.1 &      &      &     \\
SDSSJ0737+4825 & 07:37:08.71 +48:25:51.2 &      &      &     \\
ULASJ0743+2457 & 07:43:52.61 +24:57:43.6  &     22$\pm$4  & -  & - \\
SDSSJ0746+4403 & 07:46:53.04 +44:03:51.3 &      &      &     \\
SDSSJ0806+2006 & 08:06:23.68 +20:06:31.5  &     27$\pm$5  & -  & - \\
SDSSJ0818+0601 & 08:18:30.43 +06:01:37.6  &    161$\pm$5  &     48$\pm$5  & - \\
   HS0818+1227 & 08:21:38.90 +12:17:30.9 &      &      &     \\
ULASJ0820+0812 & 08:20:16.09 +08:12:16.8  &    107$\pm$4  & -  & - \\
SDSSJ0832+0404 & 08:32:17.06 +04:04:04.4 &      &      &     \\
    J0907+0003 & 09:07:10.49 +00:03:21.2 &      &      &     \\
    J0941+0518 & 09:41:22.54 +05:18:23.8  &    113$\pm$4  &     70$\pm$4  & - \\
SDSSJ0946+1835 & 09:46:04.84 +18:35:40.3  &     33$\pm$4  & -  & - \\
SDSSJ1029+2623 & 10:29:13.84 +26:23:30.2 &      &      &     \\
SDSSJ1054+2733 & 10:54:40.89 +27:33:06.1  &     32$\pm$5  &    100$\pm$5  & - \\
SDSSJ1055+4628 & 10:55:45.45 +46:28:39.7 &      &      &     \\
SDSSJ1128+2402 & 11:28:18.49 +24:02:17.4  &     51$\pm$4  &     85$\pm$4  & - \\
SDSSJ1131+1915 & 11:31:57.79 +19:15:27.4  &     35$\pm$4  & -  & - \\
SDSSJ1226$-$0006 & 12:26:08.02 $-$00:06:02.2  &     31$\pm$4  &     32$\pm$4  & - \\
SDSSJ1254+1857 & 12:54:40.34 +18:57:12.0  &    226$\pm$18  & -  & - \\
SDSSJ1254+2235 & 12:54:19.00 +22:35:36.0 &      &      &     \\
SDSSJ1258+1657 & 12:58:19.24 +16:57:17.6  &     52$\pm$4  &     69$\pm$4  & - \\
SDSSJ1304+2001 & 13:04:43.60 +20:01:05.0  &     25$\pm$4  &     16$\pm$4  & - \\
SDSSJ1320+1644 & 13:20:59.47 +16:44:03.7  &    123$\pm$5  &     22$\pm$5  & - \\
SDSSJ1334+3315 & 13:34:01.39 +33:15:34.3 &      &      &     \\
SDSSJ1339+1310 & 13:39:07.20 +13:10:39.0  &     25$\pm$5  &     20$\pm$5  & - \\
SDSSJ1349+1227 & 13:49:29.93 +12:27:07.7  &     49$\pm$4  &    160$\pm$4  & - \\
SDSSJ1353+1138 & 13:53:06.34 +11:38:04.7  &     79$\pm$4  &     32$\pm$4  & - \\
ULASJ1405+0959 & 14:05:15.44 +09:59:29.8  &     37$\pm$4  &     48$\pm$4  &     23$\pm$4 \\
SDSSJ1442+4055 & 14:42:54.70 +40:55:35.6  &     64$\pm$5  &     38$\pm$5  & - \\
SDSSJ1452+4224 & 14:52:11.50 +42:24:29.6 &      &      &     \\
SDSSJ1455+1447 & 14:55:01.88 +14:47:34.8  &     63$\pm$4  & -  & - \\
SDSSJ1458$-$0202 & 14:58:47.62 $-$02:02:05.3 &      &      &     \\
SDSSJ1515+1511 & 15:15:38.54 +15:11:35.1  &     70$\pm$12  &     61$\pm$12  & - \\
ULASJ1527+0141 & 15:27:20.22 +01:41:40.1 &      &      &     \\
ULASJ1529+1038 & 15:29:38.89 +10:38:04.3 &      &      &     \\
    J1616+1415 & 16:16:46.42 +14:15:43.9 &      &      &     \\
SDSSJ1620+1203 & 16:20:26.23 +12:03:40.7  &    327$\pm$6  & -  & - \\
    J1623+7533 & 16:23:16.92 +75:33:17.3 &      &      &     \\
  PSJ1640+1045 & 16:40:18.17 +10:45:05.4 &      &      &     \\
  PSJ1831+5447 & 18:31:27.12 +54:47:59.6  &    777$\pm$9  &    553$\pm$9  &   2429$\pm$9 \\
    J1949+7732 & 19:49:36.28 +77:32:39.0  &     39$\pm$5  &     50$\pm$5  & - \\
  PSJ2124+1632 & 21:24:16.85 +16:32:17.2  &     27$\pm$4  &     22$\pm$4  & - \\
 HE2149$-$2745 & 21:52:07.46 $-$27:31:49.4  &     45$\pm$5  & -  & - \\
   HS2209+1914 & 22:11:30.30 +19:29:12.8  &    384$\pm$4  &    459$\pm$4  & - \\
  A2213$-$2652 & 22:13:38.38 $-$26:52:27.1  &     25$\pm$5  & -  & - \\
    J2250+2117 & 22:50:34.49 +21:17:24.0  &    149$\pm$8  & -  & - \\
    J2257+2349 & 22:57:25.37 +23:49:30.4 &      &      &     \\
  PSJ2305+3714 & 23:05:55.78 +37:14:20.8  &     23$\pm$4  &     31$\pm$4  & - \\
  PSS2322+1944 & 23:22:07.16 +19:44:23.0  &     16$\pm$4  &     38$\pm$4  & - \\
WISE2329$-$1258 & 23:29:57.84 $-$12:58:59.0  &    150$\pm$5  &    139$\pm$5  &    215$\pm$5 \\
PSJ2332$-$1852 & 23:32:19.32 $-$18:52:06.6  &     59$\pm$11  &    125$\pm$11  &     59$\pm$11 \\
ULASJ2343$-$0050 & 23:43:11.94 $-$00:50:34.3  &     36$\pm$4  & -  & - \\
    J2350+3654 & 23:50:07.54 +36:54:34.5 &      &      &     \\

